Generating Human Motion in 3D Scenes from Text Descriptions

Generating human motions from textual descriptions has gained growing research interest due to its wide range of applications. However, only a few works consider human-scene interactions together with text conditions, which is crucial for visual and physical realism. This paper focuses on the task of generating human motions in 3D indoor scenes given text descriptions of the human-scene interactions. This task presents challenges due to the multi-modality nature of text, scene, and motion, as well as the need for spatial reasoning. To address these challenges, we propose a new approach that decomposes the complex problem into two more manageable sub-problems: (1) language grounding of the target object and (2) object-centric motion generation. For language grounding of the target object, we leverage the power of large language models. For motion generation, we design an object-centric scene representation for the generative model to focus on the target object, thereby reducing the scene complexity and facilitating the modeling of the relationship between human motions and the object. Experiments demonstrate the better motion quality of our approach compared to baselines and validate our design choices.

==> figures/figure_chatgpt.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/ChatGPT.pdf}
    
    \caption{\protect\textbf{Pipeline of localizing the target object.}
    In stage 1, given the input text description and detected object bounding boxes (bbx), we construct the first prompt asking \protect\chatgpt{} the categories of target objects and anchor objects. Based on the response, the scene graph can be simplified. In stage 2, we construct the second prompt with inputs and results from stage 1, including object relations derived from the simplified scene graph. The second prompt is designed for asking \protect\chatgpt{} to infer the target object. Finally, we can get the target object bounding box from the response of \protect\chatgpt{}.
    }
    \label{fig:chatgpt}
\end{figure*}

==> figures/figure_overview.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Overview.pdf}
    
    \caption{\protect\textbf{Overview of our two-stage pipeline.} 
    In the first stage, given an input scene and a text description (a), we use \protect\chatgpt{} to locate the target object (b). 
    In the second stage, human motions are synthesized by first producing human trajectories (c) and then generating local poses (d).
    }
    \label{fig:overview}
\end{figure*}

==> figures/figure_prox.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\linewidth]{figures/PROX.pdf}

    \caption{\protect\textbf{Qualitative results of our method on the PROX dataset.}
    We run our method on the scenes from the PROX dataset without fine-tuning.
    Results show that our method is capable to generalize to unseen scenes and objects.
    }
    \label{fig:prox}
\end{figure}

==> figures/figure_quality.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figures/Quality.pdf}    

    \caption{\protect\textbf{Qualitative results.} 
    We compare our method with groundtruth and four baselines (please refer to \protect\secref{sec:compare}) given the same text descriptions. 
    Our method synthesizes motions that interact with the object precisely as the groundtruth data while the baselines fail.}
    
    \label{fig:quality}
\end{figure*}
